Product of Tensors and Description of Networks

Any kind of network can be naturally represented by a Directed Acyclic Graph (DAG); additionally, activation functions can determine the reaction of each node of the network with respect to the signal(s) incoming. We study the characterization of the signal distribution in a network under the lens of tensor algebra. More specifically, we describe every activation function as tensor distributions with respect to the nodes, called \textit{activation tensors}. The distribution of the signal is encoded in the \textit{total tensor} of the network. We formally prove that the total tensor can be obtained by computing the \textit{Batthacharya-Mesner Product} (BMP), an $n$-ary operation for tensors of order $n$, on the set of the activation tensors properly ordered and processed via two basic operations, that we call \textit{blow} and \textit{forget}. Our theoretical framework can be validated through the related code developed in Python.

==> Sections/biblio.tex <==
\begin{thebibliography}{TKMPP}

\bibitem{B} P. Bhattacharya. \emph{A new 3-D transform using a ternary product}. IEEE Trans. on Signal Proc. vol.43 (1995), 3081-3084. 
\bibitem{BM1} P. Bhattacharya, D.M. Mesner. \emph {Association schemes on triples and a ternary algebra.}  J. Comb. Theory A vol.55 (1990), 204-234.
\bibitem{BM2} P. Bhattacharya, D.M. Mesner. \emph {A ternary algebra arising from an association scheme on triples.} J. Algebra vol.164 (1994), 595-613.
\bibitem{BC} C. Bocci, L. Chiantini. \emph{ An Introduction to Algebraic Statistic With
Tensors}. Unitext, Springer International Publishing  (2019).
\bibitem{DI} R. Diestel. \emph{Graph Theory.} Graduate Texts in Mathematics Springer, Heidelberg. New York, Fourth edition (2010).
\bibitem{G} E.K. Gnang. \emph{A combinatorial approach to hypermatrix algebra.} Preprint arXiv 1403.3134 (2014).
\bibitem{GF1} E.K. Gnang, Y. Filmus. \emph{On the spectra of hypermatrix direct sum and kronecker products constructions.}  vol.519 (2017), 238–277.
\bibitem{GF2} E.K. Gnang, Y. Filmus. \emph{On the Bhattacharya-Mesner rank of third order hypermatrices.} Lin. Algebra Applic. vol.588 (2020), 391–418.
\bibitem{H} L. Hogben. \emph{Handbook of linear algebra.} CRC press, 2013.
\bibitem{M} S. Marziali, \emph{Boolean Operators and Neural Networks}. Preprint (2023).
\bibitem{TKMP} F. Tian, M.E. Kilmer, E. Miller, A. Patra. \emph{ Tensor BM-Decomposition for Compression and Analysis of Spatio-Temporal Third-order Data.} Preprint arXiv 2306.09201 (2023).
\bibitem{ZA}Zapata-Carratala, C., \& Arsiwalla, X. D. (2022). \emph{An Invitation to Higher Arity Science}. arXiv preprint arXiv:2201.09738.
\end{thebibliography}

